RainSD: Rain Style Diversification Module for Image Synthesis Enhancement using Feature-Level Style Distribution

Autonomous driving technology nowadays targets to level 4 or beyond, but the researchers are faced with some limitations for developing reliable driving algorithms in diverse challenges. To promote the autonomous vehicles to spread widely, it is important to address safety issues on this technology. Among various safety concerns, the sensor blockage problem by severe weather conditions can be one of the most frequent threats for multi-task learning based perception algorithms during autonomous driving. To handle this problem, the importance of the generation of proper datasets is becoming more significant. In this paper, a synthetic road dataset with sensor blockage generated from real road dataset BDD100K is suggested in the format of BDD100K annotation. Rain streaks for each frame were made by an experimentally established equation and translated utilizing the image-to-image translation network based on style transfer. Using this dataset, the degradation of the diverse multi-task networks for autonomous driving, such as lane detection, driving area segmentation, and traffic object detection, has been thoroughly evaluated and analyzed. The tendency of the performance degradation of deep neural network-based perception systems for autonomous vehicle has been analyzed in depth. Finally, we discuss the limitation and the future directions of the deep neural network-based perception algorithms and autonomous driving dataset generation based on image-to-image translation.

==> trainiou.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=none
},
tick pos=both,
title={IoU during training},
x grid style={darkgray176},
xlabel={Epoch},
xmin=-2.95, xmax=83.95,
xtick style={color=black},
y grid style={darkgray176},
ylabel={IoU},
ymin=0.417342284321785, ymax=0.616718372702598,
ytick style={color=black}
]
\addplot [orange, mark=+, mark size=3, mark options={solid}]
table {%
1 0.42640483379364
5 0.513723313808441
10 0.56364232301712
15 0.527571201324463
20 0.520628929138184
25 0.60199111700058
30 0.603411197662354
35 0.577725410461426
40 0.584530234336853
45 0.581609964370728
50 0.607655823230743
55 0.604674279689789
60 0.592810392379761
65 0.583972275257111
70 0.572862386703491
75 0.586271584033966
80 0.567368030548096
};
\addlegendentry{IoU during training}
\end{axis}

\end{tikzpicture}

